Variational Quantum Simulation of Partial Differential Equations: Applications in Colloidal Transport

We assess the use of variational quantum imaginary time evolution for solving partial differential equations. Our results demonstrate that real-amplitude ansaetze with full circular entangling layers lead to higher-fidelity solutions compared to those with partial or linear entangling layers. To efficiently encode impulse functions, we propose a graphical mapping technique for quantum states that often requires only a single bit-flip of a parametric gate. As a proof of concept, we simulate colloidal deposition on a planar wall by solving the Smoluchowski equation including the Derjaguin-Landau-Verwey-Overbeek (DLVO) potential energy. We find that over-parameterization is necessary to satisfy certain boundary conditions and that higher-order time-stepping can effectively reduce norm errors. Together, our work highlights the potential of variational quantum simulation for solving partial differential equations using near-term quantum devices.

==> misc <==
We assess the use of variational quantum imaginary time evolution to solve partial differential equations. Our results demonstrate that real-amplitude ans\"atze with full circular entangling layers lead to higher fidelity solutions compared to those with partial or linear entangling layers. To efficiently encode impulse functions, we propose a graphical mapping technique for quantum states that often requires only a single bit-flip of a parametric gate. As a proof of concept, we solve the Smoluchowski equation for colloidal deposition on a planar wall, including the Derjaguin-Landau-Verwey-Overbeek (DLVO) potential energy as a component of the Hamiltonian. We find that over-parameterization may be necessary to satisfy certain boundary conditions and that higher-order time-stepping can effectively reduce norm errors. Together, our study highlights the potential of variational quantum simulation for solving partial differential equations using near-term quantum devices.




\fy{1. Anything to add to introduction?
2. Journal recommendations?}\dax{what's a good colloidal physics journal}\fy{There is no such thing as a 'good' colloidal physics journal -- they all suck. }\fy{Can this pass for a "quantum" journal? Or just aim to arxiv it in limbo first?}
\weibin{relevant top 10\% CiteScore 2020 journals for consideration
"International Journal of Numerical Methods for Heat and Fluid Flow"
"International Journal for "Numerical Methods in Engineering"
"Quantum Science and Technology"
""
}
\fy{Dax, what do you make of "Quantum Science and Technology"? What are the odds?}
\dax{Not sure; may not be that high but we could try.
Other similar alternatives are \href{https://www.nature.com/npjqi/}{npj Quantum}, \href{https://quantum-journal.org/}{Quantum}}
\dax{I guess a relevant question here is whether the goal of this paper is (i) to communicate to the PDE/colloidal physics community and let them know about this new `alternative' quantum way of solving the Smoluchowski equation, or (ii) to communicate to the quantum community and make them aware of this new application of variational quantum simulation. If (ii) is our goal, then I think we could try \href{https://iopscience.iop.org/journal/2058-9565}{``Quantum Science and Technology"}}\fy{It is quite difficult to tell which is the more appreciative audience. For a mediocre dish like this, chef's take is to serve each diner alternately in turn and see their food reviews.}
\dax{Ok, the alternating strategy sounds fine to me.}

%--------------------------------------------------


\renewcommand{\thetable}{B\arabic{table}}
\setcounter{table}{0}
\begin{table}[!ht]

\begin{center}
\begin{tabular}{ |c|c|c|c|c| } 
\hline
\multirow{2}{7em}{Input state at $R_Y^\ast(\pi)$ layer} & \multicolumn{4}{c|}{Output state with $R_Y^\ast(\pi)$ in layer} \\
\cline{2-5}
& $\boldsymbol{l}$ & $\boldsymbol{l-1}$ & $\boldsymbol{l-2}$ & $\boldsymbol{l-3}$ \\ 
\hline
$\ket{0001}$ & $\ket{1110} = \ket{14}$ & $\ket{1011} = \ket{11}$ & $\ket{1000} = \ket{8}$ &  $\ket{\textbf{1001}} = \ket{\textbf{9}}$\\
\hline
$\ket{0010}$ & $\ket{1111} = \ket{15}$ & $\ket{0101} = \ket{5}$ & $\ket{0011} = \ket{3}$ &  $\ket{0001} = \ket{1}$\\
\hline
$\ket{0100}$ & $\ket{1101} = \ket{13}$ & $\ket{1010} = \ket{10}$ & $\ket{0110} = \ket{6}$ &  $\ket{0010} = \ket{2}$\\
\hline
$\ket{1000}$ & $\ket{1001} = \ket{9}$ & $\ket{0111} = \ket{7}$ & $\ket{1100} = \ket{12}$ &  $\ket{0100} = \ket{4}$\\
\hline
\end{tabular}
\caption{Lookup table for $R_Y^\ast(\pi)$ which encodes $\ket{x}$ in the computational basis with cardinality $\left|\left\{\ket{\boldsymbol{x}}=\bigotimes_i^4\ket{x_i}\right\}\right| = 16$. \fy{16/16 states.}
\dax{do you mean 15/15 states?}
}
\label{table:B1}
\end{center}

\begin{center}
\begin{tabular}{ |c|c|c|c|c|c| } 
\hline
\multirow{2}{7em}{Input state at $R_Y^\ast(\pi)$ layer} & 
\multicolumn{5}{c|}{Output state with $R_Y^\ast(\pi)$ in layer}
\\
\cline{2-6}
& $\boldsymbol{l}$ & $\boldsymbol{l-1}$ & $\boldsymbol{l-2}$ & $\boldsymbol{l-3}$ & $\boldsymbol{l-4}$
\\ 
\hline
$\ket{00001}$ & $\ket{30}$ & $\ket{10}$ & $\ket{6}$ &  $\ket{2}$ &  $\ket{\textbf{31}}$ \\
\hline
$\ket{00010}$ & $\ket{31}$ & $\ket{20}$ & $\ket{12}$ &  $\ket{4}$ &  $\ket{\textbf{29}}$ \\
\hline
$\ket{00100}$ & $\ket{29}$ & $\ket{11}$ & $\ket{24}$ &  $\ket{8}$ &  $\ket{\textbf{25}}$ \\
\hline
$\ket{01000}$ & $\ket{25}$ & $\ket{22}$ & $\ket{19}$ &  $\ket{16}$ &  $\ket{\textbf{17}}$ \\
\hline
$\ket{10000}$ & $\ket{17}$ & $\ket{15}$ & $\ket{5}$ &  $\ket{3}$ &  $\ket{1}$ \\
\hline
\end{tabular}
\caption{A lookup table for $R_Y^\ast(\pi)$ which encodes $\ket{x}$ in the computational basis $\left\{\ket{\boldsymbol{x}}=\bigotimes_i^5\ket{x_i}\right\}$. \fy{21/31 states(!)}. \fy{Damn. It seems like mapping trick does not cover the entire computational basis for $n=5$. Why? I dun get it. @Dax There should be an underlying math basis behind this, maybe some of those \emph{light cone} stuff we see in some of those ansatz papers? \emph{Enlighten} us! }}
\label{table:B2}
\end{center}

\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c|c|c| } 
\hline
\multirow{2}{7em}{Input state at $R_Y^\ast(\pi)$ layer} & 
\multicolumn{11}{c|}{Output state with $R_Y^\ast(\pi)$ in layer}
\\
\cline{2-12}
& $\boldsymbol{l}$ & $\boldsymbol{l-1}$ & $\boldsymbol{l-2}$ & $\boldsymbol{l-3}$ & $\boldsymbol{l-4}$ & $\boldsymbol{l-5}$ & $\boldsymbol{l-6}$ &$\boldsymbol{l-7}$ &$\boldsymbol{l-8}$ &$\boldsymbol{l-9}$ & $\boldsymbol{l-10}$
\\ 
\hline
$\ket{000001}$ & $\ket{62}$ & $\ket{43}$ & $\ket{25}$ &  $\ket{54}$ & $\ket{18}$ & $\ket{14}$ & $\ket{59}$ & $\ket{40}$ & $\ket{24}$ & $\ket{8}$ & $\ket{\textbf{57}}$\\
\hline
$\ket{000010}$ & $\ket{63}$ & $\ket{21}$ & $\ket{50}$ &  $\ket{47}$ & $\ket{36}$ & $\ket{28}$ & $\ket{53}$ & $\ket{19}$ & $\ket{48}$ & $\ket{16}$ & $\ket{\textbf{49}}$\\
\hline
$\ket{000100}$ & $\ket{61}$ & $\ket{42}$ & $\ket{39}$ &  $\ket{29}$ & $\ket{11}$ & $\ket{56}$ & $\ket{41}$ & $\ket{38}$ & $\ket{35}$ & $\ket{32}$ & $\ket{\textbf{33}}$\\
\hline
$\ket{001000}$ & $\ket{57}$ & $\ket{23}$ & $\ket{13}$ &  $\ket{58}$ & $\ket{22}$ & $\ket{51}$ & $\ket{17}$ & $\ket{15}$ & $\ket{5}$ & $\ket{3}$ & $\ket{1}$\\
\hline
$\ket{010000}$ & $\ket{49}$ & $\ket{46}$ & $\ket{26}$ &  $\ket{55}$ & $\ket{44}$ & $\ket{37}$ & $\ket{34}$ & $\ket{30}$ & $\ket{10}$ & $\ket{6}$ & $\ket{2}$\\
\hline
$\ket{100000}$ & $\ket{33}$ & $\ket{31}$ & $\ket{52}$ &  $\ket{45}$ & $\ket{27}$ & $\ket{9}$ & $\ket{7}$ & $\ket{60}$ & $\ket{20}$ & $\ket{12}$ & $\ket{4}$\\
\hline
\end{tabular}
\caption{A lookup table for $R_Y^\ast(\pi)$ which encodes $\ket{x}$ in the computational basis $\left\{\ket{\boldsymbol{x}}=\bigotimes_i^6\ket{x_i}\right\}$. \fy{63/63 states.}. \fy{Separately I checked $n=7$ and found the states repeat on the 18th layer so that means 127/127 states, so the trick seems to work for $n=6,7$. Still doesn't explain why $n=5$ failed.}}
\label{table:B3}
\end{center}
\end{table}
